This is SpArta: Rigorous Optimization of Regionally Resolved Energy Systems by Spatial Aggregation and Decomposition

Energy systems with high shares of renewable energy are characterized by local variability and grid limitations. The synthesis of such energy systems, therefore, requires models with high spatial resolution. However, high spatial resolution increases the computational effort. Here, we present the SpArta method for rigorous optimization of regionally resolved energy systems by Spatial Aggregation and decomposition. SpArta significantly reduces computational effort while maintaining the full spatial resolution of sector-coupled energy systems. SpArta first reduces problem size by spatially aggregating the energy system using clustering. The aggregated problem is then relaxed and restricted to obtain a lower and an upper bound. The spatial resolution is iteratively increased until the difference between upper and lower bound satisfies a predefined optimality gap. Finally, each cluster of the aggregated problem is redesigned at full resolution. For this purpose, SpArta decomposes the original synthesis problem into subproblems for each cluster. Combining the redesigned cluster solutions yields an optimal feasible solution of the full-scale problem within a predefined optimality gap. SpArta thus optimizes large-scale energy systems rigorously with significant reductions in computational effort. We apply SpArta to a case study of the sector-coupled German energy system, reducing the computational time by a factor of 7.5, compared to the optimization of the same problem at full spatial resolution. As SpArta shows a linear increase in computational time with problem size, SpArta enables computing larger problems allowing to resolve energy system designs with improved accuracy.

==> chapter/nom.tex <==
\newpage
\twocolumn
\section*{Nomenclature} \label{sec:nomenclature}

\noindent\textbf{Sets} \\
\noindent
\begin{tabularx}{\columnwidth}{lX}
$T$						& Time steps	\\
$\Omega$				& Scenarios		\\
$\Omega^{\mathrm{ID}}$ 	& Intraday market scenarios \\
$C$						& Capacity and energy price combinations \\
$U$						& Units						\\
$P$						& Products					\\
\end{tabularx} \\

\noindent\textbf{Variables} \\
\noindent
\begin{tabularx}{\columnwidth}{lX}
${OPEX}_t^{\mathrm{exp}}$					& Expected operational cost \\%& \SI{}{\euro} \\
${OPEX}_{t,c}^{\mathrm{price~comb}}$		& Operational cost per price combination \\%& \SI{}{\euro} \\
${OPEX}_{t,c,\omega}^{\mathrm{scenario}}$	& Operational cost per price combination and scenario \\%& \SI{}{\euro}\\
%%%
$C^{\mathrm{gas}}_{t,\omega}$	& Natural gas cost					\\%& \SI{}{\euro}\\
$R^{\mathrm{BP}}_{t,c,\omega}$	& Balancing-power market revenues	\\%& \SI{}{\euro}\\
$R^{\mathrm{DA}}_{t,\omega}$	& Day-ahead market revenues \\%& \SI{}{\euro}\\
$R^{\mathrm{ID}}_{t,\omega}$	& Intraday market revenues \\%& \SI{}{\euro}\\
%%%
$\lambda^{\mathrm{BP}}_{t,c}$	& Binary decision for price combination in the balancing-power market \\%& \multirow{2}{*}{-} \\
$\lambda^{\mathrm{DA}}_{t,\omega}$	& Binary decision to buy/sell electricity in the day-ahead market \\%& \multirow{2}{*}{-} \\
%%%%
${BUY}_{t,\omega,p}$				& Amount of bought product (e.g. natural gas)			\\%& \SI{}{\mega\watt\per\hour}\\
${DA}^{\mathrm{sell}}_{t,\omega}$	& Amount of sold electricity in the day-ahead market	\\%& \SI{}{\mega\watt\per\hour}\\
${DA}^{\mathrm{buy}}_{t,\omega}$	& Amount of purchased electricity in day-ahead market 	\\%& \SI{}{\mega\watt\per\hour}\\
%%%%
${ID}^{\mathrm{sell}}_{t,\omega}$	& Continuous intraday market trading volumes for positive flexible capacity \\%& 
${ID}^{\mathrm{buy}}_{t,\omega}$	& Continuous intraday market trading volumes for negative flexible capacity \\%& 
%%%%
${BP}^+_t$				& Amount of positive balancing power\\%& \SI{}{\mega\watt}\\
${BP}^-_t$				& Amount of negative balancing power\\%& \SI{}{\mega\watt}\\
%%%%
${P}_{u,t,\omega,p}$	& Product supply/demand of unit \\%& \SI{}{\mega\watt}\\
\end{tabularx} \\

\newpage

\noindent\textbf{Parameters} \\
\noindent
\begin{tabularx}{\columnwidth}{lX}
$\pi_{t,c,\omega}$ 									& Scenario probability \\%& - \\
$\pi^{\mathrm{BP,cp}}_{t,c,\omega}$ 				& Acceptance probability in the balancing-power market \\%& - \\
$\pi^{\mathrm{ID}}_{t,\omega}$ 	& Probability of positive or negative flexible capacity being utilized in the intraday market  \\%& 
$\pi^{\mathrm{BP,ep}}_{t,c,\omega}$					& Request probability in the balancing-power market \\%& -\\			
%%%
$\mathrm{M}^{\mathrm{BP}}$		& Big M (large number) \\%& - \\
$\mathrm{M}^{\mathrm{DA}}$		& Big M (large number) \\%& - \\
$p^{\mathrm{gas}}_t$			& Natural gas price \\%& \SI{}{\euro\per\mega\watt\per\hour} \\
$p^{\mathrm{DA, sell}}_t$		& Day-ahead market selling price \\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$p^{\mathrm{DA, buy}}_t$		& Day-ahead market purchasing price \\%& \SI{}{\euro\per\mega\watt\per\hour}\\	
${cp}^+_{t,c}$					& Positive capacity price \\%& \SI{}{\euro\per\mega\watt}\\
${cp}^-_{t,c}$					& Negative capacity price \\%& \SI{}{\euro\per\mega\watt}\\
${ep}^+_{t,c}$					& Positive energy price \\%& \SI{}{\euro\per\mega\watt\per\hour}\\
${ep}^-_{t,c}$					& Negative energy price \\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$s^{\mathrm{cp}+}_{\omega}$		& Binary parameter for acceptance of positive balancing power \\%& - \\
$s^{\mathrm{cp}-}_{\omega}$		& Binary parameter for acceptance of negative balancing power \\%& - \\
$s^{\mathrm{ep}+}_{\omega}$		& Binary parameter for request of positive balancing power \\%& - \\
$s^{\mathrm{ep}-}_{\omega}$		& Binary parameter for request of negative balancing power \\%& - \\
$s^{\mathrm{sell}}_{\omega}$	& Binary parameter to sell in the continuous intraday market \\%& - \\
$s^{\mathrm{buy}}_{\omega}$		& Binary parameter to buy in the continuous intraday market \\%& - \\
%%%%
$d_{p,t}$						& Product demand \\%& \SI{}{\mega\watt}\\
%%%%
${opt}^{\mathrm{sell}}_t$		& Option price for positive flexible capacity \\%& \SI{}{\euro\per\mega\watt}\\
${opt}^{\mathrm{buy}}_t$		& Option price for negative flexible capacity \\%& \SI{}{\euro\per\mega\watt}\\
${mc}_t$						& Marginal electricity cost \\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$u_t$							& Up-movement \\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$d_t$							& Down-movement \\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$\mu_t$ 						& Price drift \\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$\sigma_t$						& Price volatility \\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$N_t$							& Number of trading opportunities \\%& - \\
$S_t^\mathrm{ini}$				& Initial price-level				\\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$S_{t,k}$						& Last prices						\\%& \SI{}{\euro\per\mega\watt\per\hour}\\
$\Phi^\mathrm{sell}$			& Option value for positive flexible capacity at the end of the trading session \\%& 
$\Phi^\mathrm{buy}$				& Option value for negative flexible capacity at the end of the trading session \\%& 
\end{tabularx} \\

\newpage 
\onecolumn
